Improving the Robustness of Quantized Deep Neural Networks to White-Box Attacks using Stochastic Quantization and Information-Theoretic Ensemble Training

Most real-world applications that employ deep neural networks (DNNs) quantize them to low precision to reduce the compute needs. We present a method to improve the robustness of quantized DNNs to white-box adversarial attacks. We first tackle the limitation of deterministic quantization to fixed ``bins'' by introducing a differentiable Stochastic Quantizer (SQ). We explore the hypothesis that different quantizations may collectively be more robust than each quantized DNN. We formulate a training objective to encourage different quantized DNNs to learn different representations of the input image. The training objective captures diversity and accuracy via mutual information between ensemble members. Through experimentation, we demonstrate substantial improvement in robustness against $L_\infty$ attacks even if the attacker is allowed to backpropagate through SQ (e.g., > 50\% accuracy to PGD(5/255) on CIFAR10 without adversarial training), compared to vanilla DNNs as well as existing ensembles of quantized DNNs. We extend the method to detect attacks and generate robustness profiles in the adversarial information plane (AIP), towards a unified analysis of different threat models by correlating the MI and accuracy.

==> 2_related.tex <==
\section{Related Work}

In this section, we will briefly touch upon defenses found in the existing literature that have inspired the development of our defense.

\textbf{Ensemble defense.} The core idea behind ensemble defense is to combine strength from multiple models to enhance overall robustness collectively. \cite{strauss2017ensemble} explores ensemble methods by initializing models with different weights to improve robustness. \cite{pang2019improving} talks about training strategy to train diverse sets of ensemble models. \cite{sen2020empir} ensembles quantized DNN models with different numerical precision. \cite{tramr2018ensemble} introduces ensemble adversarial training, a technique that augments training data with perturbations transferred from other models. \cite{abbasi2017robustness} propose to use an ensemble of diverse specialists based on a confusion matrix. \cite{he2017adversarial} combines multiple weak defenses and concludes that it is insufficient to create a more robust defense. \cite{liu2018towards} introduce a defense algorithm called Random Self Ensemble (RSE) that enhances the security of neural networks by adding random noise to layers and ensemble predictions, effectively defending against gradient-based attacks while maintaining predictive capability without significant memory overhead. \cite{papernot2016distillation} introduces a defensive mechanism called defensive distillation to reduce the effectiveness of adversarial samples on DNNs.


\textbf{Quantization defense.} Quantization aims to reduce the precision of Neural network weights and activation. In the quantization process, the network has a sparse representation of features or weights.\cite{gholami2021survey} survey talks about recent advances and techniques used to quantize DNN in training and post-training. \cite{zhou2020neural} use rate-distortion theory to determine the most significant bits in feature representation. \cite{yang2019quantization} presents a low-bit differentiable quantization function, which can be learned in a lossless and end-to-end manner for any weight and activation. \cite{raghavan2017bitnet} introduces a knowledge distillation way of training a low-precision network. The low-precision networks obtained after quantization have robustness characteristics against adversarial attacks. \cite{lin2019defensive} introduces a defensive quantization by controlling the Lipschitz constant of the network. \cite{khalid2019qusecnets} presents a trainable quantization method to make a pre-trained network robust to attacks. \cite{rakin2018defend} proposes adaptive quantization techniques to quantize activation functions. \cite{gui2019model} introduces the Adversarially Trained Model Compression (ATMC) framework, which unifies various compression techniques (pruning, factorization, quantization) into a single constrained optimization formulation.


\textbf{Adversarial attack detection.} Attack detection refers to identifying adversarial attacks on the DNNs. It can also be considered as OOD distribution detection. \cite{bagnall2017training} proposes an ensemble method for detecting and classifying adversarial attacks. \cite{feinman2017detecting} uses Bayesian uncertainty estimates in the feature spaces to find artifacts in learned space. \cite{metzen2017detecting} trains a small detector sub-network for binary classification problems to distinguish between clean and adversarial data. \cite{wang2021multi} propose a MultiExpert Adversarial Attack Detection (MEAAD) approach by checking context inconsistency, suitable for any DNN-based ReID systems. \cite{xiang2021patchguard++} uses a small receptive field of CNNs to detect attacks in feature space. \cite{smith2018understanding} use measure of uncertainty, i.e., Mutual information, to detect attacks. \cite{lee2018simple} proposes a unified framework to detect OOD and adversarial samples using Gaussian discriminant analysis and applies it to any pre-trained softmax neural classifier. \cite{carlini2017adversarial} evaluates various attack detection algorithms and provides guidelines for evaluation. 

% \note{Adversarial attack detection.} 
% \begin{itemize}
%     % \item Training ensembles to detect adversarial example \cite{bagnall2017training}
%     % \item Detecting adversarial samples from artifacts \cite{feinman2017detecting}
%     % \item On detecting adversarial perturbations \cite{metzen2017detecting}
%     % \item Multi-Expert Adversarial Attack Detection in Person Re-identification Using Context Inconsistency \cite{wang2021multi}
%     % \item PATCHGUARD++: EFFICIENT PROVABLE ATTACK DETECTION AGAINST ADVERSARIAL PATCHES \cite{xiang2021patchguard++}
%    %  \item Understanding Measures of Uncertainty for Adversarial Example Detection \cite{smith2018understanding}
%    %  \item A simple unified framework for detecting out-of-distribution samples and adversarial attacks \cite{lee2018simple}
%      \item Adversarial examples are not easily detected: Bypassing ten detection methods \cite{carlini2017adversarial}
%     % \item Exploiting Multi-Object Relationships for Detecting Adversarial Attacks in Complex Scenes \cite{Yin_2021_ICCV}
% \end{itemize}


% List of Contribution: 
% \begin{itemize}
%    \item Proposed a SQ which is unbiased in Expectation and Generalizes to arbitrary %\#bins 
%    \item MI can calculated w/o training 
%        \begin{itemize}
%            \item We show how the SQ can be used as an instance MI estimator
%            \item What kind of distribution? 
%        \end{itemize}
%    \item End-2-End training method which optimizes CE, MI, inorder to find %compression representation which have high accuracy 
%\end{itemize}


% Results Contrib.: 
%    
%    - Tool for studying adv attacks 
%    - Evaluating MI for Adv attack; allows smooth interpolation between the attacks %of different strength 
%        - its a better interpolation; accuracy vs eps! 
%        - provides multiple bengs:
%            - compare differnt attacks types and strength 
%    
%    - Estimated MI; 
%    - imporved results for: 
%        - Attack Detection using MI 
%        - Robustness improvement (not SOTA) - Not a major outcome 
%        
%    - Message: 
%            - Maybe no general solution; 
%            - tool to see quickly where the different attacks falling 
%            - Can lead to additional insights thn just accuracy 
%            
%    - We also show tha information theoretic view is not completly solving the %problem 
%    while it is a good measure of generalization; but doesnt work universally 
%    
%    - We evaluate existing bounds on DL under our framework; 
%        - bound holds for indistibution testset 
%        - while its useless for OOD 
%        
%In the experiments: 
%    what are the positive and negs you want to highlights

%-------------------------------------------------------------------------

%%%%%%%%% Related Work

% \section{Related Work}
% \label{sec:related work}
% \subsection{Ensemble Adversarial Defenses}


% \subsection{Quantization Defenses}
% \subsection{Adversarial attack detection}

% \begin{itemize}
%   \item Cross entropy based 
%   \item MI based
%   \item Some hybrid structure 
% \end{itemize}

%------------------------------------------------------------------------

% Our work primarily extends the Randomized smoothing framework from input to features, as we call Randomized Features Smoothing. \cite{cohen2019certified}. One of the key ideas from Randomized Smoothing is that the classifier obtained after smoothing has a lower Lipschitz constant, which is primarily an indicator of an adversarial defense  \cite{finlay2018lipschitz}. Our moving defense draws inspiration from previously known ensemble-based defenses, the diversity of ensembles is a key idea to develop our ensemble which is grounded by Information theoretic properties. This Information theoretic also enables us to develop an MI estimator which can be used to develop an Adversarial detector. Next, quantization has shown to be a robust defense in the literature which converts your model to a sparse representation. Typically, this process is non-differentiable so we develop a novel differentiable Stochastic Quantization that injects controlled noise into the data distribution. All the ideas were pulled together to create our present RFS defense.

% \begin{itemize}
    % \item Ensembling via different weights initialization \cite{strauss2017ensemble}
    % \item ADP \cite{pang2019improving} 
    % \item EMPIR \cite{sen2020empir} 
    % \item Ensemble adversarial training \cite{tramr2018ensemble}
    % \item Robustness to Adversarial Examples through an Ensemble of Specialists \cite{abbasi2017robustness}
    % \item Adversarial Example Defenses: Ensembles of Weak Defenses are not Strong \cite{he2017adversarial}
    % \item Improving Adversarial Robustness via Promoting Ensemble Diversity \cite{pmlr-v97-pang19a}
    % \item Towards robust neural networks via random self-ensemble \cite{liu2018towards}
    % \item Distillation as a defense to adversarial perturbations against deep neural networks \cite{papernot2016distillation}
    % \item EOT \cite{athalye2018synthesizing}
    
% \end{itemize}

% \begin{itemize} 
%     \item Latest quantization methods: \cite{gholami2021survey}
%     \item A survey on methods and theories of quantized neural networks \cite{guo2018survey}
%     \item bitnet \cite{raghavan2017bitnet}
%     \item Neural Network Activation Quantization with Bitwise Information Bottlenecks \cite{zhou2020neural}
%     \item Quantization networks \cite{yang2019quantization}
% \end{itemize}/

% \note{Quantization Defenses}
% \begin{itemize}
%     \item Qu-ANTI-zation: Exploiting Quantization Artifacts for Achieving Adversarial Outcomes \cite{hong2021quantization}
% %     \item Defensive quantization \cite{lin2019defensive}
%  %   \item Qusecnets: Quantization-based defense mechanism for securing deep neural network against adversarial attacks \cite{khalid2019qusecnets}
%     
%  % \item Defend deep neural networks against adversarial examples via fixed and dynamic quantized activation functions \cite{rakin2018defend}
%     % \item Model Compression with Adversarial Robustness: A Unified Optimization Framework \cite{gui2019model}
%     
% \end{itemize}
